Long Document Summarization in a Low Resource Setting using Pretrained Language Models

Abstractive summarization is the task of compressing a long document into a coherent short document while retaining salient information. Modern abstractive summarization methods are based on deep neural networks which often require large training datasets. Since collecting summarization datasets is an expensive and time-consuming task, practical industrial settings are usually low-resource. In this paper, we study a challenging low-resource setting of summarizing long legal briefs with an average source document length of 4268 words and only 120 available (document, summary) pairs. To account for data scarcity, we used a modern pretrained abstractive summarizer BART (Lewis et al., 2020), which only achieves 17.9 ROUGE-L as it struggles with long documents. We thus attempt to compress these long documents by identifying salient sentences in the source which best ground the summary, using a novel algorithm based on GPT-2 (Radford et al., 2019) language model perplexity scores, that operates within the low resource regime. On feeding the compressed documents to BART, we observe a 6.0 ROUGE-L improvement. Our method also beats several competitive salience detection baselines. Furthermore, the identified salient sentences tend to agree with an independent human labeling by domain experts.

==> sections/related.tex <==
\section{Related Work}
Several recent works have focused extensively on the task of abstractive summarization. 
%Two step: \citet{gehrmann-etal-2018-bottom} proposes a bottom-up content selector to over-determine phrases within a document that are likely to appear in its summary. This is then followed 
%Long documents: Deep Communicating Agents for Abstractive Summarization
%Saliency: Multi-Reward Reinforced Summarization with Saliency and Entailment, Soft Layer-Specific Multi-Task Summarization with Entailment and Question Generation, Fast Abstractive Summarization with  Reinforce-Selected Sentence Rewriting
